Generalized Linear Bandits with Limited Adaptivity

We study the generalized linear contextual bandit problem within the constraints of limited adaptivity. In this paper, we present two algorithms, $\texttt{B-GLinCB}$ and $\texttt{RS-GLinCB}$, that address, respectively, two prevalent limited adaptivity settings. Given a budget $M$ on the number of policy updates, in the first setting, the algorithm needs to decide upfront $M$ rounds at which it will update its policy, while in the second setting it can adaptively perform $M$ policy updates during its course. For the first setting, we design an algorithm $\texttt{B-GLinCB}$, that incurs $\tilde{O}(\sqrt{T})$ regret when $M = \Omega( \log{\log T} )$ and the arm feature vectors are generated stochastically. For the second setting, we design an algorithm $\texttt{RS-GLinCB}$ that updates its policy $\tilde{O}(\log^2 T)$ times and achieves a regret of $\tilde{O}(\sqrt{T})$ even when the arm feature vectors are adversarially generated. Notably, in these bounds, we manage to eliminate the dependence on a key instance dependent parameter $\kappa$, that captures non-linearity of the underlying reward model. Our novel approach for removing this dependence for generalized linear contextual bandits might be of independent interest.

==> preamble.tex <==
\usepackage{amsmath,amsthm,mathtools,amssymb}
\usepackage{thmtools,thm-restate}
\RequirePackage{algorithm}
% \RequirePackage[noend]{algorithmic}
% \usepackage{algorithm}
\usepackage{algorithmic}
% \usepackage[usenames,svgnames,xcdraw,table]{xcolor}
% \definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
% \definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
% \usepackage{hyperref}
% \hypersetup{
%    colorlinks   = true,
%  linkcolor    = DarkBlue, % color of internal links
%  urlcolor     = DarkBlue, % color of external links
% 	 citecolor    = DarkGreen % color of links to bibliography
% }
% \usepackage[capitalize]{cleveref}
% \usepackage{graphicx}
% \usepackage{svg}
% \usepackage{float}
% % \usepackage{verbatim}
% \usepackage{caption}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{claim}[lemma]{Claim}
% \newtheorem{corollary}[lemma]{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{observation}{Observation}
% \newtheorem*{example}{Example}
% \newtheorem{remark}{Remark}
% \newtheorem{proposition}[lemma]{Proposition}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%%%%%%%%%%%%%%%%%%%%%%%THEOREMS

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem*{lemma*}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%MACROS
\newcommand{\f}[1]{\boldsymbol{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\fl}[1]{\mathbf{#1}}
\newcommand{\ca}[1]{\mathcal{#1}}
\newcommand{\m}[1]{\mathrm{#1}}
\newcommand{\s}[1]{\mathsf{#1}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\Su}{\mathsf{occ}}
\newcommand{\pj}[1]{\todo{PJ: #1}}
\newcommand{\lr}[1]{{\left|\left|#1\right|\right|}}
\newcommand{\bproof}{\bigskip {\bf Proof. }}
\newcommand{\eproof}{\hfill\qedsymbol}
\newcommand{\fac}{\Phi}
\newcommand{\welf}{\textsc{Wel-Alg}}
\newcommand{\alg}{\textsc{Alg}}
\newcommand{\Ttil}{\widetilde{\s{T}}}
\newcommand{\Td}{\s{T}'}
\newcommand{\T}{\s{T}}
\newcommand{\x}{\mathbf x}
\newcommand{\bX}{\mathbf X}
\newcommand{\bV}{\mathbf V}
\newcommand{\bA}{{\mathbf A}}
\newcommand{\bI}{{\mathbf I}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bG}{{\mathbf G}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\cX}{{ \mathcal{X}}}

\newcommand{\ctX}{\widetilde{{ \mathcal{X}}}}
\newcommand{\cE}{{ \mathcal{E}}}
\newcommand{\cA}{{ \mathcal{A}}}
\newcommand{\cB}{{ \mathcal{B}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\enet}{{ \mathcal{C}}_\varepsilon}
\newcommand{\opt}{\bm{\omega}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\arm}{\mathtt{arm}}
\newcommand{\thta}{\theta^*}
\newcommand{\thth}{\widehat{\theta}}
\newcommand{\thtill}{\widetilde{\theta}}
\DeclareMathOperator*{\E}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\NRg}{\textsc{NR}}
\newcommand{\Rg}{\textsc{R}}
\newcommand{\ex}{\mathrm{exp}}
\newcommand{\LNCB}{\mathrm{LNCB}}
\newcommand{\UNCB}{\mathrm{UNCB}}
\newcommand{\UCB}{\mathrm{UCB}}
\newcommand{\Sample}{S}
\newcommand{\norm}[2]{\left\lVert #1 \right\rVert_{#2}}
\newcommand{\sfT}{\s{T}}
\newcommand{\cvx}{\mathrm{cvh}}
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
\newcommand{\lrc}[1]{\left\{ #1 \right\}}
\newcommand{\lrb}[1]{\left[ #1 \right]}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}


\newcommand{\dotprod}[2]{\langle #1 ,#2 \rangle}
% \newcommand{\dotprod}[2]{ #1^\T #2 }
\newcommand{\bd}{\dot{b}}
\newcommand{\bdd}{\Ddot{b}}
\newcommand{\bddd}{\dddot{b}}
\newcommand{\mud}{\dot{\mu}}
\newcommand{\mudd}{\ddot{\mu}}
\newcommand{\xtil}{\widetilde{x}}
\newcommand{\ytil}{\widetilde{y}}
\newcommand{\mudp}[2]{\mud \left( \dotprod{#1}{#2} \right) }
\newcommand{\mup}[2]{\mu \left( \dotprod{#1}{#2} \right) }
\newcommand{\kap}{\kappa}
\newcommand{\kapst}{{\kappa^*}}
\newcommand{\kapav}{{\widehat{\kappa}}}
\newcommand{\const}{\textbf{c}}
%\newcommand{\detCond}{(1 + \textbf{ f })}
\newcommand{\detCond}{2}
\newcommand{\batchAlgoName}{\texttt{B-GLinCB}}
\newcommand{\rarelyAlgoName}{\texttt{RS-GLinCB}}
\newcommand{\contextualbandit}{\texttt{CB}}
\newcommand{\linearcontextualbandit}{\texttt{LinCB}}
\newcommand{\genlinearcontextualbandit}{{\texttt{GLinCB}}}
\newcommand{\Reg}{\textsc{R}}
\newcommand{\reg}{\textbf{reg}}

\def\DEBUG{true} % set this to be false to remove comments
	\ifdefined\DEBUG
\newcommand{\gaurav}[1]{{\footnotesize\color{red}[Gaurav: #1]}}
\newcommand{\ayush}[1] {{\footnotesize\color{orange}[AS: #1]}}
\newcommand{\siddharth}[1] {{\footnotesize\color{brown}[Siddharth: #1]}}
\newcommand{\nirjhar}[1] {{\footnotesize\color{cyan}[Nirjhar: #1]}}
\newcommand{\gopt}{\textsc{G-optimal design} }
\newcommand{\dopt}{\textsc{Distributional optimal design} }

\newcommand{\bluetext}[1]{{\color{blue} #1}}

\newcommand{\redtext}[1]{{\color{red} #1}}
%%Alg line label fix
\newcommand{\alglinelabel}{%
  \addtocounter{ALC@line}{-1}% Reduce line counter by 1
  \refstepcounter{ALC@line}% Increment line counter with reference capability
  \label% Regular \label
}
